Prompting as Probing: Using Language Models for Knowledge Base Construction

Language Models (LMs) have proven to be useful in various downstream applications, such as summarisation, translation, question answering and text classification. LMs are becoming increasingly important tools in Artificial Intelligence, because of the vast quantity of information they can store. In this work, we present ProP (Prompting as Probing), which utilizes GPT-3, a large Language Model originally proposed by OpenAI in 2020, to perform the task of Knowledge Base Construction (KBC). ProP implements a multi-step approach that combines a variety of prompting techniques to achieve this. Our results show that manual prompt curation is essential, that the LM must be encouraged to give answer sets of variable lengths, in particular including empty answer sets, that true/false questions are a useful device to increase precision on suggestions generated by the LM, that the size of the LM is a crucial factor, and that a dictionary of entity aliases improves the LM score. Our evaluation study indicates that these proposed techniques can substantially enhance the quality of the final predictions: ProP won track 2 of the LM-KBC competition, outperforming the baseline by 36.4 percentage points. Our implementation is available on https://github.com/HEmile/iswc-challenge.

==> main_backup.tex <==
% This is samplepaper.tex, a sample chapter demonstrating the
% LLNCS macro package for Springer Computer Science proceedings;
% Version 2.20 of 2017/10/04
%
% \documentclass[runningheads]{llncs}
%
\usepackage{graphicx}
\renewcommand{\arraystretch}{1.25}


\usepackage{wrapfig}
\usepackage{todonotes}
%\usepackage[disable]{todonotes}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{url}
\usepackage{paralist}
\usepackage{booktabs}

\usepackage{hyperref}
\usepackage{cleveref}

\usepackage{draftwatermark}
\SetWatermarkText{BACKUP COPY}
\SetWatermarkScale{4.5}

% Used for displaying a sample figure. If possible, figure files should
% be included in EPS format.
%
% If you use the hyperref package, please uncomment the following line
% to display URLs in blue roman font according to Springer's eBook style:
% \renewcommand\UrlFont{\color{blue}\rmfamily}

\begin{document}
%
\title{Prompting as Probing: Large Language Models for Knowledge Base Construction}
%
\titlerunning{Prompting as Probing: LLMs for KB Construction}
% If the paper title is too long for the running head, you can set
% an abbreviated paper title here
%
\author{First Author\inst{1}\orcidID{0000-1111-2222-3333} \and
Second Author\inst{2,3}\orcidID{1111-2222-3333-4444} \and
Third Author\inst{3}\orcidID{2222--3333-4444-5555}}
%
\authorrunning{F. Author et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{Vrije Universiteit, Amsterdam, Netherlands \and
Universiteit van Amsterdam, Amsterdam, Netherlands}
%
\maketitle              % typeset the header of the contribution
%
\begin{abstract}
High-capacity, pre-trained Large Language Models (LLMs) and the word representations (embeddings) they provide have proven to be useful in a variety of downstream tasks and are becoming increasingly important in our field. In parallel, they have shown great results when \textit{prompted} in the right way. In this work, we utilize one of the largest and most powerful, publicly queryable, LLMs to date called GPT-3 by OpenAI, to perform the task of Knowledge Base Construction (KBC). 
We present a modular approach that combines a variety of LLM-based to perform KBC.
In our extensive evaluation, we demonstrate how our different components balance out each other's weaknesses ensuring high-quality triple completions.

%Our results show that the LLM is able to perform the task and is able to outperform the baselines by 40\%.
\todo[inline]{MC: I would not include results in the abstract just yet. We could consider it for the camera ready.}

\keywords{Language models  \and Knowledge Base Completion \and Prompt engineering.}
\end{abstract}
%
% A system description in PDF format (5-12 pages, LNCS style).
%
\section{Introduction}
% LLM overview
Large Language Models (LLMs) have been at the center of media attention, presented as a recent success story of Artificial Intelligence. 
Rising popularity aside, LLMs have shown great promise in a variety of different tasks (e.g. Classification, Financial Sentiment Analysis, and even Protein Binding Site Prediction \cite{daza2021inductive,araci2019finbert,elnaggar2020prottrans}) in a variety of domains (e.g. Biomedical). 
Investigating the full capabilities/potential of said LLMs is becoming a research field itself, with a plethora of papers working on LLM understanding (see \Cref{sec:related_work} for more related work).

One of the questions researchers have recently investigated, is whether LLMs have the potential to be used as Knowledge Bases.
% Researchers recently investigated the question, whether could be used as knowledge graphs. 
In the seminal paper by Petroni et al. \cite{petroni2019language}, the LAMA dataset, a dataset for probing relational facts from Wikidata in LLMs was presented.
The authors show that the masked LLM BERT can complete Wikidata facts with a precision of around 32\%.
Several follow-up papers have pushed this number to almost 50\%~\cite{zhang2022opt,qin-eisner-2021-learning}.
While the prediction quality on LAMA is promising, it was argued that LMs should not be used as knowledge graphs, but rather to support the augmentation and curation of KGs~\cite{razniewski2021language}.

% The task
In this report, we discuss the system we implemented for the Knowledge Base Construction from Pre-trained Language Models (LM-KBC) challenge\footnote{\url{https://lm-kbc.github.io/}}, at ISWC 2022. 
This submission is in Track 2, where language models of any size can be used. 
The task is to predict possible objects of a triple, where the subject and relation are given.
For example, given the string "Ronnie James Dio" as the subject and the relation \textit{PersonInstrument}, one needs to predict the strings "bass guitar" or "guitar", and "trumpet", as the objects of the triple.
Different from what has been done in previous works, e.g. in LAMA, is that the number of entities to be predicted can be multiple, as in the example, but also zero.
Since a set of results is expected, the evaluation is done using precision and recall metrics rather than the more common ranking-based measures
\todo[inline]{Shameless self cite? https://arxiv.org/abs/2102.11389  -- it is not really spot on, but about the same issue. JC:  LAMA also uses ranking metrics and is probably more related, but I don't wanna steal your citation

MC: the point is that the paper I would cite is arguing for precision/recall metrics rather than ranking based. But, the context is query answering, rather than question answering/completion in this fashion.
}

% Formally, given the input subject-entity (s) and relation (r), the task is to predict all the correct object-entities ({o1, o2, ..., ok}) using LM probing.


% What are we doing? Prompt Engineering 
In our system, we make use of the GPT3 model, hosted by OpenAI. 
For each relation type, we engineered prompts that, when given to the language model, probe it to respond with the set of objects. 
\todo[inline]{MC Add one-two sentences about specifics like voting, etc. JC: We need to put the different components here!}

% Observation
We found out that using this approach, we get high-quality predictions. 
\todo[inline]{JC: No results here? I would at least add our final number at the end of the introduction}
Besides, in several of the cases where the result was counted as incorrect, the ground truth was either incomplete or used aliases with the same meaning.
Overall, we conclude that language models can certainly be used to augment knowledge bases, that the evaluation of this type of task is rather hard, and that more investigation and theoretical understanding are required to decide whether language models can be a replacement for knowledge bases built from text.


\section{Related Work}
\label{sec:related_work}
% LM for AKBC - Jan

The development of large pre-trained language models has led to substantial improvements in NLP research.
It was shown that an extensive pre-training on large text corpora, encodes large amounts of linguistic and factual knowledge into a language model that can help to improve the performance on various downstream tasks.
Recently, it was discussed how far language models can replace (\cite{petroni2019language}) or support the creation and curation of knowledge graphs (\cite{razniewski2021language}).


\textbf{LM as KG}
Petroni et al. \cite{petroni2019language} asked the question "Language Models as Knowledge Bases?".
They proposed the LAMA dataset for probing relational knowledge in language models by using masked language models to complete cloze-style % this is not a spelling issue: cloze
sentences. 
As an example, the language model BERT can complete the sentence ``Paris is the capital of [MASK]" with the word ``France".
In this case, it is assumed that the model \textit{knows} about, or is able to predict, the triple (Paris, capitalOf, France).

While the original paper relied on manually designed prompts for probing the language model, various follow-up works have shown the superiority of automatically learning prompts.
Methods can either mine prompts from large text corpora and pick the best prompts by applying them to a training dataset as demonstrated in~\cite{jiang2020how,bouraoui2020inducing}.
Prompts can also be directly learned via backpropagation.
BERTESE and AutoPrompt show how discrete prompts can be learned to improve the performance on LAMA~\cite{shin2020autoprompt,haviv-etal-2021-bertese}.
The probing performance can be even pushed further by either directly learning continuous embeddings for the prompts~\cite{qin-eisner-2021-learning,zhong2021factual} or by directly fine-tuning the LM on the training data~\cite{fichtel2021prompt}.

Similar to our work, in FewShot-LAMA few-shot learning on the original LAMA dataset is evaluated~\cite{he2021an}.
The authors show that a combination of few-shot examples with learned prompts achieves the best probing results.

Since the publication of the LAMA dataset, a large variety of other probing datasets for factual knowledge in LMs have been created.
LAMA-UHN is a more difficult version of LAMA~\cite{poerner2019bert}. 
TimeLAMA adds a time component to facts that the model is probed for~\cite{dhingra2021time}.
Besides, BioBERT and MedBERT are domain-specific probing datasets for biological and medical knowledge~\cite{sung2021can,meng2021rewire}.



Most existing approaches have in common that they only probe the language models for entities with a label consisting of a single token from the language model's vocabulary.
Thus, the prediction of long, complex entity names is largely unexplored.
Furthermore, most existing works have only asked language models to complete a triple with a single prediction, even though some triples might actually allow for multiple possible predictions.
Both these aspects make this challenge on knowledge graph construction substantially different.


\textbf{LM for KG}
While probing language models has been heavily studied in the NLP community, the idea of using language models to support knowledge graph curation is not sufficiently studied~\cite{razniewski2021language}.
Some works have shown how LMs in combination with knowledge graphs can be used to complete query results~\cite{kalo2020b}.
Another work has looked into how to use language models for identifying errors in knowledge graphs~\cite{arnaout2022utilizing}.
Other works have looked into weighting KG triples, i.e., facts from ConceptNet with language models to measure semantic similarity.
Biswas et al. have shown that language models can be used to perform entity typing by predicting the class using language models~\cite{biswas2021do}.

KG-BERT is a system that is most similar to what is required for the KBC competition\cite{yao2019kgbert}. 
A standard BERT model is trained on serialized knowledge graph data to perform link prediction on standard link prediction benchmark datasets.
KG-BERT is performing similarly well for link prediction as many state-of-the-art systems that are based on knowledge graph embeddings.

\todo{JC: should we leave this here or integrate it somewhere else? I think it could be integrated in the part where we present our prompts}
% Similar tasks 
\textbf{Similar tasks}
This task is similar to Factual Q\&A with Language models, where the goal is to respond to questions that fall outside of a knowledge base. This shared task differs in that the responses need to include 0 to k answers. Moreover, in the shared task, the factual questions are generated from triples, thus including variation in how a triple might be phrased as a question.


\section{The Challenge}


% Zero or more entities may be predicted as the tail for a triple, 
% \todo[inline]{MC the following part of the sentence is unclear to me. }
% while one or several aliases may be given for each of these tail entities. 

We are given a dataset with triples of the form $(s, p, O)$, where $s$ signifies textual representation of the \textit{subject}, $p$ signifies on of 12 different predicates and $O$ the (possibly empty) set of textual representations of \textit{object} entities for prediction. 
The subjects and objects are of various entity types. 
\newline

\noindent After learning from a training set of such triples, given a new subject and one of the known relations, the task is to predict the complete set of objects. 

\subsection{Data}
% \todo[inline]{JC: I think it would be nice to have some sentences giving an overview over the dataset here}
\label{sec:data}
For each of the 12 relations, the number of unique subject-entities in the train, dev, and test are 100, 50, and 50. We include detailed distributions of the number of object-entities per relation type (Appendix, \Cref{fig:train_set_stats,fig:dev_set_stats}). \Cref{tab:answer_count_averages} include aggregated statistics related to the number of object-entities, and the number of alternative labels per object-entities in the development set. In the rest of this section we discuss characteristics and patterns we found while working with this dataset.

\begin{table}[]
\centering
\caption{Dataset statistics  regarding the number of object-entities, and alternative labels per object-entity, per relation}
\label{tab:answer_count_averages}
\scriptsize{
\begin{tabular}{lrr}
\toprule
                          & \multicolumn{2}{c}{\emph{\#object-entities}}                         \\ \cline{2-3} 
                          & \multicolumn{1}{c}{\emph{mean}} & \multicolumn{1}{c}{\emph{std}} \\ \midrule
\textbf{Relation Type}                  &                          &                         \\ \midrule
CompanyParentOrganization & 0.32                 & 0.47                \\ \hline
PersonPlaceOfDeath        & 0.50                 & 0.51                \\ \hline
PersonCauseOfDeath        & 0.52                 & 0.54                \\ \hline
PersonLanguage            & 1.70                 & 1.18                \\ \hline
PersonInstrument          & 1.86                 & 2.81                \\ \hline
CountryOfficialLanguage   & 2.06                 & 2.47                \\ \hline
PersonEmployer            & 2.14                 & 1.65                \\ \hline
RiverBasinsCountry        & 2.28                 & 1.67                \\ \hline
ChemicalCompoundElement   & 3.38                 & 1.12                \\ \hline
CountryBordersWithCountry & 4.04                 & 2.69                \\ \hline
StateSharesBorderState    & 5.62                 & 2.92                \\ \hline
PersonProfession          & 7.42                 & 4.85                \\ \bottomrule
\end{tabular}
}
\end{table}

%\todo[inline]{TT Table is missing a description. I would round the numbers in Table 1 up or down to two decimal places.}


\subsubsection{Cardinality differences among relations}
From \Cref{tab:answer_count_averages} we see that some relations have a much higher average cardinality (e.g. \textit{PersonProfession}=7.42 or \textit{StateSharesBorderState}=5.6) than others (\textit{CompanyParentOrganization}=0.32, \textit{PersonPlaceOfDeath}=0.50). We hypothesize that relations with a larger standard deviation for the number of object-entities, will be harder to predict.

We also note that only five of the relations allow for empty answer sets. For example, relations associated with a person's death (\textit{PersonPlaceOfDeath} and \textit{PersonCauseOfDeath}) often contain empty values, because many persons in the dataset are still alive.  In these cases, it would be important for a method to be able to predict NONE correctly. %it is highly likely that a model that just learns to predict death or not death (NONE vs something) might be the cause to go from 0.3 to 0.7.

\subsubsection{Alternative labels}
\todo[inline]{JC: I am a bit confused by the idea of the data section. The previous subsection was about data statistics, while this is about the shortcomings of the dataset. I would try to separate this differently.}
This task does not include entity linking. 
Instead, predicted entities are scored against a list of their aliases. 
However, we noticed these lists are often incomplete. 
For example, for the "National Aeronautics and Space Administration", the extremely common and widely used abbreviation "NASA", is not included in the list of aliases.
Another example occurs when the model predicts Aluminum (US and Canadian English) where the ground truth only has Aluminium (English in the rest of the world), a lower score gets obtained.
Hence, if the model predicts Aluminum or Nasa, the predictions are deemed incorrect.
 % Arnold S as language Austrian German which has alias German

\subsubsection{Contemporaneity of LLMs}
Another important finding that came up during our analysis, was related to how up-to-date the model is i.e. how recent were the data used to train the model. 
We observed that models that were trained for example until 2019, would fail in most cases involving facts that happened later on, such as in 2020. 
This falls in line with related findings around LLMs and is further confirmed as a finding by OpenAI\footnote{\url{https://beta.openai.com/docs/guides/embeddings/limitations-risks}}.

% Language models are trained in a specific point in time. Any facts that change overtime are thus prone to errors. 

In our experimentation we found, for example, that the GPT3 model trained in June 2021 makes mistakes related to the fact that "Facebook" had changed their name to "Meta" (in October 2021), that Harry Styles learned how to play piano after he became famous (2013), and that the country of "Swaziland" changed its name to "Eswatini" (2018). 
Note that it is not important when the model was trained, but rather whether the corpus the model is trained on contains the up-to-data information.
% information about people's deaths after this is not known by the model

\subsection{Baseline}
As a baseline, the competition organisers provided us with a masking-based approach that uses the well-studied BERT model \cite{devlin2018bert} in 3 variants (\emph{base-cased},\emph{large-cased} and \emph{RoBERTa} \cite{liu2019roberta}).
From our initial observations of the baseline performance, we found that recall tends to be higher than precision, which differs from the results of our process which is analysed in the following section.
\todo[inline]{JC: THe last sentence confuses me. Isn't the precision high and recall low? And what exactly is "analysed in the following section"? Because the results are not. }


\section{Our Method}
Previous studies have shown that prompt formulation plays a critical role in the performance of LMs on downstream applications \cite{reynolds2021prompt} and similarly, this also applies to our work. We investigated different prompting approaches using few-shot learning with GPT-3\ \cite{brown2020language} using OpenAI’s API \footnote{https://openai.com/api (temperature=0, max\_tokens=100, top\_p=1, frequency\_penalty=0, presence\_penalty=0, logprobs=1)}. In this Section, we describe how we generate the prompts, and how we utilise different components in our pipeline to further fine-tune the prompts for an enhanced performance. 

% \todo[inline]{JC: This should mention the "components" that we prominently advertised in abstract and intro.}

% \todo[inline]{JC: Does it make sense to not mention the triple prompts here already? It is a bit weird reading about how manually curated prompts, even though this is only half of what we used in the end.}

% \todo[inline]{LM or LLM? We need to make sure that this is consistently used throughout the paper.}

\subsection{Prompt Generation}

For each relation in the dataset, we manually curate a set of prompt templates consisting of four representative examples \footnote{This is an arbitrary number of training examples. Since few-shot learners are efficient at learning from a handful of examples \cite{brown2020language}, including excessive number of training examples may not necessarily lead to any improved precision or recall. Therefore, we did not study the effects of varying the number of training examples in the prompts.} selected from the training split. We use these relation-specific templates to generate prompts for every subject entity by replacing a placeholder token in the final line of the template with the subject entity of interest. GPT-3 is tasked with completing the prompts, and we evaluate the \emph{completions} and compute the macro-precision, macro-accuracy and macro-F1 score for each relation.

We ensured that the training examples for few-shot learning met all of the following requirements: 
\begin{inparadesc}
\item[Questions with answer sets of variable lengths] to inform the LM that it can generate multiple answers, 
\item[Empty answer sets] to ensure that the LM returns nothing when there is no correct answer to a given question, 
\item[Fixed Question-Answer Order] i.e., we provide the question and then immediately the answer so that the LM learns the style of the format, and 
\item[Answer set formatted as a list] to ensure we can efficiently parse the answer set from the LM.
\end{inparadesc}

We formulate the questions either in natural language or in the form of a triple. In the former case, we present the questions in natural language (\emph{e.g.} \verb|Where is or was Susan Wojcicki employed?|) and then provide the correct answers as a list on the next line \verb|['Google']|. In the latter case, we use the triple format \verb|subject predicate: object| to phrase the question and give the answer on the same line (\emph{e.g.} \verb|Susan Wojcicki PersonEmployer: ['Google']|). The prompt templates are shown in Section \ref{prompt-appendix} in the Appendix. In our work, we investigate the use of both prompting styles and compare natural language prompts with triple-based prompts for the different relations. 

\subsection{Empty Answer sets}

There some questions in the dataset for which the correct answer is an empty answer set. For instance, \emph{there are no countries that share borders with the country Fiji}. The empty answer set can be represented as either an empty list \verb|[]|, or as a string within a list \verb|['None']|, and we have observed that the way that empty set are represented affects the precision and recall of our approach. We believe that by explicitly including 'None' encourages the LM exclude answers that it is uncertain about.

\subsection{Fact probing}
Our initial results indicated that the recall of our approach was high but the precision for certain relations were low. 
Therefore, we consider an additional step in our pipeline where we ask the GPT-3 to probe the truthfulness of a completion. We call it \emph{fact probing}. This was inspired by maieutic prompting \cite{jung2022maieutic}, which selects a correct answer to a question from noisy and inconsistent generations of LMs by asking questions which results in a TRUE or FALSE. We use a simple prompt where we translate each prompt into a natural language fact, and ask the model to predict whether this fact is true or false. We ensure GPT-3 only predicts either \verb|TRUE| or \verb|FALSE| by giving both a true and a false example.

% \subsubsection{Prompt Paraphrasing}
% Paraphrasing aims to improve upon lexical diversity while remaining relatively faithful to the original prompt" (from How Can We Know What Language Models Know


\section{Results}
In this section we describe the effect of each of the decisions we made for this challenge. In the end, we combine the best-performing hyper-parameters to make a final submission and compare against the baseline. 

\subsection{Ameliorating the predictions}

\subsubsection{Natural language vs triple based prompt}
We first want to identify whether putting efforts into creating prompts would be fruitful, or if simply putting the triple information would suffice. We note that most relations (7 out of 12) do better when using a simple triple based prompt. 

% predictions/gpt3(davinci-dev-language-empty).pred.jsonl
\begin{table*}[h]
\centering
\scriptsize{
\caption{
\label{table:results_per_rel_davinci_triple} Performance over relation types comparing triple vs natural language formatting for prompts.}
\begin{tabular}{|p{4.5cm}|p{1cm}|p{1.2cm}|p{1cm}|p{1.2cm}|p{1cm}|p{1.2cm}|}
\hline
\textbf{Relation Type}  & \multicolumn{2}{|c|}{\textbf{Precision}} & \multicolumn{2}{|c|}{\textbf{Recall}} & \multicolumn{2}{|c|}{\textbf{F1}} \\ \hline
\textbf{Method}  & Triple     & Natural Language  & Triple     & Natural Language  & Triple     & Natural Language  \\ \hline
ChemicalCompoundElement   & \underline{0.976} & 0.895 & \underline{0.919} & 0.885 & \underline{0.940} & 0.884 \\ \hline
CompanyParentOrganization & \underline{0.627} & 0.385 & \underline{0.640} & 0.400 & \underline{0.630} & 0.388 \\ \hline
CountryBordersWithCountry & \underline{0.865} & 0.809 & 0.733 & \underline{0.800} & 0.766 & \underline{0.785} \\ \hline
CountryOfficialLanguage   & \underline{0.933} & 0.798 & 0.810 & \underline{0.882} & \underline{0.833} & 0.785 \\ \hline
PersonCauseOfDeath        & \underline{0.560} & 0.500 & \underline{0.550} & 0.500 & \underline{0.553} & 0.500 \\ \hline
PersonEmployer            & 0.261 & \underline{0.273} & 0.267 & \underline{0.323} & 0.226 & \underline{0.262} \\ \hline
PersonInstrument          & \underline{0.547} & 0.489 & \underline{0.508} & 0.458 & \underline{0.502} & 0.446 \\ \hline
PersonLanguage            & \underline{0.840} & 0.750 & 0.894 & \underline{0.932} & \underline{0.827} & 0.793 \\ \hline
PersonPlaceOfDeath        & 0.820 & \underline{0.840} & 0.820 & \underline{0.840} & 0.820 & \underline{0.840} \\ \hline
PersonProfession          & 0.669 & \underline{0.713} & 0.527 & \underline{0.535} & 0.556 & \underline{0.581} \\ \hline
RiverBasinsCountry        & \underline{0.845} & 0.820 & 0.868 & \underline{0.863} & \underline{0.832} & 0.822 \\ \hline
StateSharesBorderState    & \underline{0.587} & 0.628 & 0.407 & \underline{0.462} & 0.472 & \underline{0.522} \\ \hline
\hline
\textbf{** Average over all relations **} & 0.711 & 0.658 & 0.662 & 0.657 & 0.663 & 0.634 \\ \hline
\end{tabular}}
\end{table*}

\subsubsection{Empty vs None}
Five out of twelve relations allow for \emph{None} answers. We experiment on which representation would yield the best results with this specific type of prediction.  LLMs seem to have an inherent weakness in predicting empty lists/strings. We note that 2 relations get a performance boost prompted with 'NONE' (\textit{CompanyParentOrganization}, \textit{PersonCauseOfDeath}), while the other three relations perform better when using empty lists (\textit{CountryBordersWithCountry}, \textit{PersonInstrument}, \textit{PersonPlaceOfDeath}). For subsequent experiments, we modified the prompt of each relation to use the best performant representation. 

% predictions/gpt3(davinci-dev-empty).pred.jsonl
\begin{table*}[h]
\centering
\scriptsize{
\caption{
\label{table:results_per_rel_davinci_empty} Performance over relation types for \textit{da-vinci-002} with \textit{empty results} allowed.}
\begin{tabular}{|p{5cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
\hline
\textbf{Relation Type}  & \multicolumn{2}{|c|}{\textbf{Precision}} & \multicolumn{2}{|c|}{\textbf{Recall}} & \multicolumn{2}{|c|}{\textbf{F1}} \\ \hline
\textbf{Method}  & []     & ['None']  & []     & ['None']  & []     & ['None']  \\ \hline
CompanyParentOrganization & 0.485 & \underline{0.685} & 0.500 & \underline{0.700} & 0.488 & \underline{0.688} \\ \hline
CountryBordersWithCountry & \underline{0.830} & 0.815 & \underline{0.794} & 0.782 & \underline{0.792} & 0.778 \\ \hline
PersonCauseOfDeath        & 0.560 & \underline{0.580} & 0.560 & \underline{0.580} & 0.560 & \underline{0.580} \\ \hline
PersonInstrument          & \underline{0.589} & 0.545 & \underline{0.570} & 0.520 & \underline{0.551} & 0.519 \\ \hline
PersonPlaceOfDeath        & \underline{0.820} & 0.800 & \underline{0.820} & 0.800 & \underline{0.820} & 0.800 \\ \hline
\hline
\textbf{** Average over all relations **} & 0.685 & \underline{0.697} & 0.674 & \underline{0.685} & 0.657 & \underline{0.669} \\ \hline
\end{tabular}}
\end{table*}

\subsubsection{Language Model Size}
% https://blog.eleuther.ai/gpt3-model-sizes/
% Back up the sizes of the models with a proper reference
Another experiment was dedicated on analysing the effect that different model sizes have on the task of KBC. Our hypothesis lies on the basis of related findings, that want LLMs be more performant when larger in size, almost independently of the downstream task at hand. Specifically in our case, we are interested on whether the \textit{larger} the LLM in terms of embedding dimensionality for its tokens, the \textit{better} the performance on KBC. Figure \ref{fig:performance_per_model_type} shows our results. From a set of 4 different models with different embedding sizes, we can see that as the language model size increases, performance follows along.


\begin{figure*}[ht!]
    \centering
    \includegraphics[trim={0 0 0 0},clip,width=\linewidth]{img/performance_per_model_size.pdf}
    \caption{\label{fig:performance_per_model_type}Performance of models with different embedding sizes. We can observe an almost analogous increase between size and performance.}
\todo[inline]{TT: we need to make the font size bigger in the figure}
\todo[inline]{MC: can someone try a log scale for the x-axis and put the models in the right place? Otherwise a trendline does not make sense.}
\end{figure*}



% \begin{table*}[h]
% \centering
% \scriptsize{
% \caption{
% \label{table:results-scaling}Experimental results.}
% \begin{tabular}{|p{5cm}|p{2cm}|p{2cm}|p{2cm}|}
% \hline
% \textbf{Method} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \hline \hline
% Baseline (BERT) & 17.51 & 12.87 & 14.02 \\ \hline
% GPT3-350M (Ada)  & 0.180  & 0.194 & 0.161 \\ \hline
% GPT3-1.3B (Babbage)  & 0.325   & 0.263 & 0.269 \\ \hline
% GPT3-6.7B (Curie)  & 0.378 & 0.375 & 0.343 \\ \hline
% GPT3-175B (Davinci)  & 0.707 & 0.694 & 0.677 \\ \hline
% OPT-1.3B  & & & \\ \hline
% OPT-6.7B   & & & \\ \hline
% OPT-13B   & & & \\ \hline
% OPT-30B   & & & \\ \hline
% \end{tabular}}
% \end{table*}

\subsection{Post-processing predictions}

\subsubsection{Fact probing}
We report performance by relation type because logic integrity has a different impact depending on the semantics and cardinality of the relation. For example, \textit{PersonPlaceOfDeath}, which has only one correct answer, should show a higher improvement than \textit{State Borders}, which has a higher cardinality (Insert here average cardinality in train and dev sets).

\begin{table*}[h]
\centering
\scriptsize{
\caption{
\label{table:results-probing}Experimental results.}
\begin{tabular}{|p{5cm}|p{2cm}|p{2cm}|p{2cm}|}
\hline
\textbf{Method} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \hline \hline
Baseline (dev) & 0.349  & 0.295  & 0.309 \\ \hline
BERT + logic integrity (dev) &  0.357 & 0.304 & 0.317 \\ \hline
\hline
GPT3-Davinci (dev) & 0.729 &	0.691 &	0.689 \\ \hline
GPT3-Davinci + logic integrity (dev) & 0.734 &	0.684 &	0.690 \\ \hline
\hline
GPT3-Davinci (test) & 0.7879 &	0.7042 &	0.6832 \\ \hline
GPT3-Davinci + logic integrity (test) & 0.8045 &	0.6936 &	0.6796 \\ \hline
\end{tabular}}
\end{table*}

\subsubsection{Ambiguity}
Similar to the previous, we find differences in the relations and the ambiguity present in the target entities. Some entities, such as countries, have an official name and thus reduced ambiguity. However, institutions, which have official names, popular names and acronyms, are more ambiguous. We  observe that adding aliases to the predictions has a larger impact on ambiguous relations.

\begin{table*}[h]
\centering
\scriptsize{
\caption{
\label{table:results-ambiguity}Experimental results.}
\begin{tabular}{|p{5cm}|p{2cm}|p{2cm}|p{2cm}|}
\hline
\textbf{Method}     & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \hline \hline
Baseline (BERT) & 17.51 & 12.87 & 14.02 \\ \hline
BERT + enriched labels  & & & \\ \hline
OUR BEST PERFORMANCE FROM PREV TABLE  & 66.92 & 67.59 & 64.61 \\ \hline
OUR BEST PERFORMANCE FROM PREV TABLE + enriched labels  & & & \\ \hline
\end{tabular}}
\end{table*}


\subsection{Entity aliases}
% \todo[inline]{MC old text, new version below\\
% When performing KBC, it is important to deal with the problem of ambiguity of the predicted \textit{object entities}. For example, if the LLM predicts the token \textit{NASA} for the \textit{Employer} of \textit{Shane Kimbrough}, but the ground truth data, only contains \textit{national aeronautics and space administration} then we observed an unreasonable performance drop. Hence, one of the prompt tuning components that we introduce in this work is using Wikidata \cite{Citewiki} to disambiguate between different aliases of the same entity in the predictions.
% }

\todo[inline]{MC there are two perspectives here. We can look at this from the perspective of KBC, where we need to know which entity it is and we need to do entity disambiguation. We can also look at it from the evaluation angle, where we notice that answers are sometime correct but not exactly the same. I am currently including both, we can remove one if desired.}

As we discussed in \Cref{sec:data}, the predictions from the language model are sometimes correct, but not according to what the gold standard expects.
Whether this is problematic depends on the final use of the predictive model. 
In interactive use, this would not be an issue because the user is able to disambiguate.
For actual KBC, one would need to disambiguate, i.e., know which exact entity is meant. 
Here, however, we only check whether the text generated by the model corresponds to one of the gold standard alternatives.

%This way of evaluating has some issues. For example, for the gold standard, one would expect aliases to be acceptable. In the development set we see, for example, both Czechia and its former name Czech Republic as acceptable answers for the Central European country. 
%However, this is rather inconsistent. For example, for the country Eswatini in Southern Africa, the former name Swaziland is not included.

While experimenting, we noticed that in the training and development set the names of entities often correspond with the labels of entities in Wikidata\footnote{\url{https://www.wikidata.org}}. 
On Wikidata, these entities also have aliases and hence, we wanted to know whether we can improve our system by looking up the aliases on Wikidata. This lookup is not making use of language models, so it is \emph{not included as part of our system}. 
Rather, we perform it as an ablation study.

We work as follows. First, we extract a set of types which could be relevant for the specific relation types. For example, country (Q6256) is relevant for \textit{RiverBasinsCountry}. Then, for each relation type, we extract all correctly typed entities, their aliases, and claim count.
Then, we take the answer predicted by the LM, and check whether there is an entity with that label for that relation. If so, we retain the answer.

If not, we check whether the prediction is equal to any of the aliases. There could be multiple entities for which this is the case. Therefore, we pick the label of the entity which has most claims on Wikidata. The assumptions are that it is more likely the answer is an interesting entity and that these interesting entities have more claims on Wikidata.

We observe that

\todo[inline]{Complete this based on the observations}


\section{Conclusion}
\todo[inline]{JC: This is a summary and not a conclusion.}
In this paper, we described thoroughly our approach to perform KBC with the use of high-capacity pre-trained LLM. We showcase how we developed different modular components that utilise both LLM and the provided data by the organisers to ameliorate our performance, such as the \textit{fact probing} and the \textit{alias fetcher} components. In an attempt to "break" the black box open, we have further investigated well-known techniques around prompt engineering and optimisation and analysed the effect of different prompt formulations on the final performance. Last but not least, we report on performance and show how our suggested approach is outperforming the baseline provided by the competition organisers by even $40\%$. 

% Future work ideas: 1) Improve fact checking, 2) have the LLM generate and optimise its own prompts
Regarding future work, a natural continuation of this work can revolve around improving the individual modules (i.e. fact checking) and their performance, which will directly reflect to the overall performance of our approach. Additionally, we could experiment with inversing the pipeline and allow the LLM to generate the best prompts by providing the ground truth as input.

In terms of additional components that make use of LLMs, we have considered developing \textit{meta-prompts} as in \cite{reynolds2021prompt}. An interesting question would be, what meta-prompts should be developed for KBC? Is there a set of specific patterns that work better than others? 
Finally, we could modify our \textit{alias-fetcher} to make use of the LLM component of our approach in order to generate well-known aliases for both entities and relations in the training data. This would act as a diversification factor and our hypothesis is that although it will not be as \emph{strong} as a dictionary-based approach, it will have a higher degree of freedom to choose aliases, making it really interesting to investigate.

\todo[inline]{TT: I moved this paragraph from Section 4 to here because we don't use this in our approach (if I understood it correctly). We should phrase it as a future work.}
Data augmentation differs from \textit{prompt tuning} in the following ways: While prompt tuning is looking for the optimal prompt to increase the performance over a specific task, \textit{data augmentation} acts simply as a diversification mechanism over our existing prompts. The hypothesis is that, by employing a more diverse set of prompts we can increase our performance, especially in terms of recall. Last but not least, we base our hypothesis on the fact that knowledge is expressed in a diverse manner (e.g. ambiguity) and we have to take that into consideration when prompting a LLM.


% Future work:
% \begin{enumerate}
%     \item Fact checking can be improved with a more advanced prompt, such as the logical integrity prompt from Maieutic prompting or language models know what it knows (see paper on slack). 
% \end{enumerate}

\paragraph*{Supplemental Material Statement:}Code and data are publicly available from
\url{https://github.com/HEmile/iswc-challenge}. 

\subsubsection{Acknowledgements}
This research was funded by the Vrije Universiteit Amsterdam and the Netherlands Organisation for Scientific Research (NWO) via the \textit{Spinoza} grant (SPI 63-260) awarded to Piek Vossen,  the \textit{Hybrid Intelligence Centre} via the Zwaartekracht grant (024.004.022), Elsevier’s Discovery Lab, and Huawei's DReaMS Lab.

%
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%
\bibliography{mybib}
\bibliographystyle{splncs04}
%
\newpage
% \appendix
\section{Appendix}

\subsection{Dataset statistics}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{img/relation_statistics_train_set.pdf}
    \caption{\#Answers per relation type for the training set provided by the organisers.}
    \label{fig:train_set_stats}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{img/relation_statistics_dev_set.pdf}
    \caption{\#Answers per relation type for the development set provided by the organisers.}
    \label{fig:dev_set_stats}
\end{figure}

\subsection{Prompts} \label{prompt-appendix}

Here, we show the templates we used to generate the prompts for the different relations. In our template, we use \verb|{subject_entity}| to refer to the head entity for which we are predicting the tail entities for. The generated prompts were used for the following models: Ada, Babbage, Curie and Davinci.

\subsubsection{CountryBordersWithCountry}

\begin{verbatim}
Which countries neighbour Dominica?
['Venezuela']

Which countries neighbour North Korea?
['South Korea', 'China', 'Russia']

Which countries neighbour Serbia?
['Montenegro', 'Kosovo', 'Bosnia and Herzegovina', 'Hungary', 
'Croatia', 'Bulgaria',  'Macedonia', 'Albania', 'Romania']

Which countries neighbour Fiji?
[]

Which countries neighbour {subject_entity}?
\end{verbatim}

\subsubsection{CountryOfficialLanguage}

\begin{verbatim}
Suriname CountryOfficialLanguage: ['Dutch']

Canada CountryOfficialLanguage: ['English', 'French']

Singapore CountryOfficialLanguage: ['English', 'Malay', 'Mandarin', 
'Tamil']

Sri Lanka CountryOfficialLanguage: ['Sinhala', 'Tamil']

{subject_entity} CountryOfficialLanguage:         
\end{verbatim}

\subsubsection{StateSharesBorderState}

\begin{verbatim}
San Marino StateSharesBorderState: ['San Leo', 'Acquaviva', 
'Borgo Maggiore', 'Chiesanuova', 'Fiorentino']

Whales StateSharesBorderState: ['England']

Liguria StateSharesBorderState: ['Tuscany', 'Auvergne-Rhoone-Alpes', 
'Piedmont', 'Emilia-Romagna']

Mecklenberg-Western Pomerania StateSharesBorderState: ['Brandenburg', 
'Pomeranian', 'Schleswig-Holstein', 'Lower Saxony']

{subject_entity} StateSharesBorderState:
\end{verbatim}

\subsubsection{RiverBasinsCountry}

\begin{verbatim}
Drava RiverBasinsCountry: ['Hungary', 'Italy', 'Austria', 
'Slovenia', 'Croatia']

Huai river RiverBasinsCountry: ['China']

Paraná river RiverBasinsCountry: ['Bolivia', 'Paraguay', 
Argentina', 'Brazil']

Oise RiverBasinsCountry: ['Belgium', 'France']

{subject_entity} RiverBasinsCountry:
\end{verbatim}

\subsubsection{ChemicalCompoundElement}

\begin{verbatim}
Water ChemicalCompoundElement: ['Hydrogen', 'Oxygen']

Bismuth subsalicylate ChemicalCompoundElement: ['Bismuth']

Sodium Bicarbonate ChemicalCompoundElement: ['Hydrogen', 'Oxygen', 
'Sodium', 'Carbon']

Aspirin ChemicalCompoundElement: ['Oxygen', 'Carbon', 'Hydrogen']

{subject_entity} ChemicalCompoundElement:
\end{verbatim}

\subsubsection{PersonLanguage}

\begin{verbatim}
Aamir Khan PersonLanguage: ['Hindi', 'English', 'Urdu']

Pharrell Williams PersonLanguage: ['English']

Xabi Alonso PersonLanguage: ['German', 'Basque', 'Spanish', 'English']

Shakira PersonLanguage: ['Catalan', 'English', 'Portuguese', 'Spanish', 
'Italian', 'French']

{subject_entity} PersonLanguage:
\end{verbatim}

\subsubsection{PersonProfession}

\begin{verbatim}
What is Danny DeVito's profession?
['Comedian', 'Film Director', 'Voice Actor', 'Actor', 'Film Producer', 
'Film Actor', 'Dub Actor', 'Activist', 'Television Actor']

What is David Guetta's profession?
['DJ']

What is Gary Lineker's profession?
['Commentator', 'Association Football Player', 'Journalist', 
'Broadcaster']

What is Gwyneth Paltrow's profession?
['Film Actor','Musician']

What is {subject_entity}'s profession?
\end{verbatim}

\subsubsection{PersonInstrument}

\begin{verbatim}
Liam Gallagher PersonInstrument: ['Maraca', 'Guitar']

Jay Park PersonInstrument: ['None']

Axl Rose PersonInstrument: ['Guitar', 'Piano', 'Pander', 'Bass']

Neil Young PersonInstrument: ['Guitar']

{subject_entity} PersonInstrument:
\end{verbatim}

\subsubsection{PersonEmployer}

\begin{verbatim}
Where is or was Susan Wojcicki employed?
['Google']

Where is or was Steve Wozniak employed?
['Apple Inc', 'Hewlett-Packard', 'University of Technology Sydney', 'Atari']

Where is or was Yukio Hatoyama employed?
['Senshu University','Tokyo Institute of Technology']

Where is or was Yahtzee Croshaw employed?
['PC Gamer', 'Hyper', 'Escapist']

Where is or was {subject_entity} employed?
\end{verbatim}

\subsubsection{PersonPlaceOfDeath}

\begin{verbatim}
What is the place of death of Barack Obama?
[]

What is the place of death of Ennio Morricone?
['Rome']

What is the place of death of Elon Musk?
[]

What is the place of death of Prince?
['Chanhassen']

What is the place of death of {subject_entity}?
\end{verbatim}

\subsubsection{PersonCauseOfDeath}

\begin{verbatim}
André Leon Talley PersonCauseOfDeath: ['Infarction']

Angela Merkel PersonCauseOfDeath: ['None']

Bob Saget PersonCauseOfDeath: ['Injury', 'Blunt Trauma']

Jamal Khashoggi PersonCauseOfDeath: ['Murder']

{subject_entity} PersonCauseOfDeath:
\end{verbatim}

\subsubsection{CompanyParentOrganization}

\begin{verbatim}
Microsoft CompanyParentOrganization: ['None']

Sony CompanyParentOrganization: ['Sony Group']

Saab CompanyParentOrganization: ['Saab Group', 'Saab-Scania', 
'Spyker N.V.', 'National Electric Vehicle Sweden'', 'General Motors']

Max Motors CompanyParentOrganization: ['None]

{subject_entity} CompanyParentOrganization:
\end{verbatim}

\subsection{Failure cases}

Here, we list three failure examples for each relation for the Davinci model. A comprehensive list of failure cases can be found under \href{https://github.com/HEmile/iswc-challenge/tree/main/failure_cases}{https://github.com/HEmile/iswc-challenge/tree/main/failure\_cases}.

\subsubsection{CountryBordersWithCountry}

\begin{verbatim}
SubjectEntity: Bahrain
Ground Truth: ['iran', 'saudi arabia']
GPT-3 Prediction: ['qatar', 'saudi arabia', 'united arab emirates']

SubjectEntity: Barbados
Ground Truth: []
GPT-3 Prediction: ['trinidad and tobago']

SubjectEntity: Cuba
Ground Truth: ['united states of america', 'usa']
GPT-3 Prediction: ['bahamas', 'haiti', 'jamaica', 
'turks and caicos islands', 'united states']
\end{verbatim}

\subsubsection{CountryOfficialLanguage}

\begin{verbatim}
SubjectEntity: Afghanistan
Ground Truth: ['arabic', 'baluchi', 'dari', 'nuristani', 'pamir', 
'pashayi', 'pashto', 'turkmen', 'uzbek']
GPT-3 Prediction: ['dari', 'pashto']

SubjectEntity: Botswana
Ground Truth: ['english']
GPT-3 Prediction: ['setswana']

SubjectEntity: Zimbabwe
Ground Truth: ['barwe', 'chewa', 'english', 'kalanga', 'khoisan', 
'nambya', 'ndau', 'ndebele', 'northern ndebele', 'sesotho', 'shona', 
'tonga', 'tsonga', 'tswana', 'venda', 'xhosa']
GPT-3 Prediction: ['chewa', 'english', 'ndebele', 'shangaan', 'shona', 
'sotho', 'tonga', 'venda']
\end{verbatim}

\subsubsection{StateSharesBorderState}

\begin{verbatim}
SubjectEntity: Andalusia
Ground Truth: ['beja', 'castile-la mancha', 'extremadura', 'faro', 
'gibraltar', 'murcia', 'region of murcia']
GPT-3 Prediction: ['castilla-la mancha', 'ceuta', 'extremadura', 
'melilla', 'murcia']

SubjectEntity: Obwalden
Ground Truth: ['canton of bern', 'canton of lucerne', 'lucerne', 
'nidwalden', 'schwyz', 'uri']
GPT-3 Prediction: ['berne', 'uri', 'valais']

SubjectEntity: Zagreb
Ground Truth: ['krapina-zagorje', 'krapina-zagorje county', 
'zagreb', 'zagreb county']
GPT-3 Prediction: ['bosnia and herzegovina', 'serbia', 'slovenia']
\end{verbatim}

\subsubsection{RiverBasinsCountry}

\begin{verbatim}
SubjectEntity: Didi Liakhvi river
Ground Truth: ['georgia']
GPT-3 Prediction: ['georgia', 'russia']

SubjectEntity: Dniester
Ground Truth: ['moldova', 'ukraine']
GPT-3 Prediction: ['moldova', 'romania', 'ukraine']

SubjectEntity: San
Ground Truth: ['poland', 'ukraine']
GPT-3 Prediction: ['mexico']
\end{verbatim}

\subsubsection{ChemicalCompoundElement}

\begin{verbatim}
SubjectEntity: Aluminum Iodide
Ground Truth: ['aluminium', 'iodine']
GPT-3 Prediction: ['aluminum', 'iodine']

SubjectEntity: Atracurium Besylate
Ground Truth: ['carbon', 'hydrogen', 'nitrogen', 'oxygen', 'sulfur']
GPT-3 Prediction: ['atracurium', 'hydrogen', 'oxygen']

SubjectEntity: Flavin Adenine Dinucleotide
Ground Truth: ['carbon', 'hydrogen', 'nitrogen', 'oxygen', 'phosphorus']
GPT-3 Prediction: ['adenine', 'dinucleotide', 'flavin']
\end{verbatim}

\subsubsection{PersonLanguage}

\begin{verbatim}
SubjectEntity: A. R. Rahman
Ground Truth: ['hindi', 'tamil', 'telugu']
GPT-3 Prediction: ['bengali', 'hindi', 'kannada', 'malayalam', 
'marathi', 'tamil', 'telugu']

SubjectEntity: Akon
Ground Truth: ['english']
GPT-3 Prediction: ['english', 'french', 'wolof']

SubjectEntity: Genelia D'Souza
Ground Truth: ['hindi', 'malayalam', 'tamil', 'telugu']
GPT-3 Prediction: ['bengali', 'english', 'hindi', 'marathi', 'telugu']
\end{verbatim}

\subsubsection{PersonProfession}

\begin{verbatim}
SubjectEntity: Elon Musk
Ground Truth: ['engineer', 'entrepreneur', 'inventor', 'programmer']
GPT-3 Prediction: ['businessperson', 'engineer', 'inventor', 
'investor', 'philanthropist', 'product designer']

SubjectEntity: J. K. Rowling
Ground Truth: ['author', "children's writer", 'executive producer', 
'film producer', 'novelist', 'producer', 'producer', 'screenwriter', 
'writer', 'writer']
GPT-3 Prediction: ['author', 'film producer', 'philanthropist', 
'screenwriter']

SubjectEntity: Lady Gaga
Ground Truth: ['singer', 'songwriter']
GPT-3 Prediction: ['actress', 'dancer', 'philanthropist', 
'record producer', 'singer', 'songwriter']
\end{verbatim}

\subsubsection{PersonInstrument}

\begin{verbatim}
SubjectEntity: Ronan Keating
Ground Truth: []
GPT-3 Prediction: ['piano']

SubjectEntity: Taeyang
Ground Truth: []
GPT-3 Prediction: ['guitar']

SubjectEntity: Chester Bennington
Ground Truth: []
GPT-3 Prediction: ['guitar', 'piano']
\end{verbatim}

\subsubsection{PersonEmployer}

\begin{verbatim}
SubjectEntity: Kent Beck
Ground Truth: ['meta platforms']
GPT-3 Prediction: ['facebook', 'three rivers institute']

SubjectEntity: Serena Williams
Ground Truth: ['unicef']
GPT-3 Prediction: ['tennis']

SubjectEntity: Guido van Rossum
Ground Truth: ['microsoft']
GPT-3 Prediction: ['dropbox', 'google']
\end{verbatim}

\subsubsection{PersonPlaceOfDeath}

\begin{verbatim}SubjectEntity: Avicii
Ground Truth: ['muscat']
GPT-3 Prediction: ['muscat, oman']

SubjectEntity: John Coltrane
Ground Truth: ['huntington']
GPT-3 Prediction: ['new york city']

SubjectEntity: Rachel Caine
Ground Truth: ['texas']
GPT-3 Prediction: ['']
\end{verbatim}

\subsubsection{PersonCauseOfDeath}

\begin{verbatim}
SubjectEntity: Ahmed Zewail
Ground Truth: ['lymphoma', 'spinal cord lymphoma']
GPT-3 Prediction: ['cancer']

SubjectEntity: Avicii
Ground Truth: ['exsanguination']
GPT-3 Prediction: ['suicide']

SubjectEntity: Ennio Morricone
Ground Truth: ['femoral fracture', 'fracture']
GPT-3 Prediction: [''] 
\end{verbatim}

\subsubsection{CompanyParentOrganization}

\begin{verbatim}
SubjectEntity: Aston Martin lagonda
Ground Truth: []
GPT-3 Prediction: ['aston martin lagonda global holdings plc']

SubjectEntity: Austro-Daimler
Ground Truth: []
GPT-3 Prediction: ['daimler ag']

SubjectEntity: Hyundai Motor Company
Ground Truth: ['hyundai']
GPT-3 Prediction: ['hyundai motor group']

\end{verbatim}

\end{document}

